From MiniZinc to Optimization Modulo Theories, and Back (Extended Version)

Optimization Modulo Theories (OMT) is an extension of SMT that allows for finding models that optimize objective functions. In this paper we aim at bridging the gap between Constraint Programming (CP) and OMT, in both directions. First, we have extended the OMT solver OptiMathSAT with a FlatZinc interface -- which can also be used as a FlatZinc-to-OMT encoder for other OMT solvers. This allows OMT tools to be used in combination with mzn2fzn on the large amount of CP problems coming from the MiniZinc community. Second, we have introduced a tool for translating SMT and OMT problems on the linear arithmetic and bit-vector theories into MiniZinc. This allows MiniZinc solvers to be used on a large amount of SMT/OMT problems. We have discussed the main issues we had to cope with in either directions. We have performed an extensive empirical evaluation comparing three state-of-the-art OMT-based tools with many state-of-the-art CP tools on (i) CP problems coming from the MiniZinc challenge, and (ii) OMT problems coming mostly from formal verification. This analysis also allowed us to identify some criticalities, in terms of efficiency and correctness, one has to cope with when addressing CP problems with OMT tools, and vice versa.

==> Makefile <==
LATEX=pdflatex
SOURCE=main
JOB_NAME=main_long

.PHONY:

default: short

all: long-bib short-bib

clean:
	$(RM) main.pdf main_long.pdf  *.ps *.dvi *.aux *.toc *.log *.bak *.backup *.blg *.bbl *.cut *~

short: set_short
	$(LATEX) --jobname=$(JOB_NAME) $(SOURCE)

short-bib: set_short
	$(LATEX) --jobname=$(JOB_NAME) $(SOURCE)
	bibtex   $(JOB_NAME)
	$(LATEX) --jobname=$(JOB_NAME) $(SOURCE)
	$(LATEX) --jobname=$(JOB_NAME) $(SOURCE)

long: set_long
	$(LATEX) --jobname=$(JOB_NAME) $(SOURCE)

long-bib: set_long
	$(LATEX) --jobname=$(JOB_NAME) $(SOURCE)
	bibtex   $(JOB_NAME)
	$(LATEX) --jobname=$(JOB_NAME) $(SOURCE)
	$(LATEX) --jobname=$(JOB_NAME) $(SOURCE)

upload:
	git push

#
# The following commands are invoked AUTOMATICALLY,
# there is no need to use any of them explicitly.
#

set_appendix: force
	bash -c 'sed -i "s/\\\\newcommand{\\\\withproofs}{true}/\\\\newcommand{\\\\withproofs}{false}/g" options.tex'

set_proofs: force
	bash -c 'sed -i "s/\\\\newcommand{\\\\withproofs}{false}/\\\\newcommand{\\\\withproofs}{true}/g" options.tex'

set_short: force
	$(eval JOB_NAME=main)
	bash -c 'sed -i "s/\\\\newcommand{\\\\longversion}{true}/\\\\newcommand{\\\\longversion}{false}/g" options.tex'

set_long: force
	$(eval JOB_NAME=main_long)
	bash -c 'sed -i "s/\\\\newcommand{\\\\longversion}{false}/\\\\newcommand{\\\\longversion}{true}/g" options.tex'

force:
	git update-index --assume-unchanged options.tex


==> src/tables/mc16.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}[tb]
\centering
\begin{tabularx}{\textwidth}{|X|r|xrrr|r|rr|}
\hline
{\bf tool, configuration \& encoding} &
{\bf inst.} &
{\bf termin.} &
{\bf timeout} &
{\bf unsup.} &
{\bf errors} &
{\bf time (s.)} &
{\bf BT1} &
{\bf BT2} \\
\hline
{\sc \gfd{}}                       & 100 & 21 & 75 &  0 & 4 &  8656 &  0 &  0\\
{\sc \picat{}(cp)}                 & 100 & 21 & 79 &  0 & 0 &  8324 &  0 &  0\\
{\sc \gecode{}()}                  & 100 & 39 & 61 &  0 & 0 & 12163 &  0 &  0\\
{\sc \choco{}()}                   & 100 & 47 & 53 &  0 & 0 & 15679 &  1 & 1\\
{\sc \izplus{}()}                  & 100 & 50 & 50 &  0 & 0 &  6491 &  7 & 7\\
{\sc \chuffed{}()}                 & 100 & 53 & 42 &  5 & 0 &  4822 &  5 & 5\\
{\sc \jacop{}()}                   & 100 & 58 & 42 &  0 & 0 & 16236 &  0 & 0\\
{\sc \ortools{}(cp)}               & 100 & 62 &  8 & 30 & 0 &  1570 & 27 & 27\\
{\sc \gurobi{}()}                  & 100 & 72 & 28 &  0 & 0 &  5382 & 15 & 15\\
{\sc \hcsp{}()}                    & 100 & 73 & 27 &  0 & 0 &  5035 & 10 & 10\\
{\sc \picat{}(sat)}                & 100 & 74 & 26 &  0 & 0 &  8637 & 11 & 11\\
{\sc \ortools{}(sat)}              & 100 & {\bf \blue{84}} & 16 &  0 & 0 & 12163 & 33 & 32\\
\hline
{\sc \vbest{}(\minizinc{})}    & 100 & 93 &  7 & 0 & 0 &  3657 & - & -\\
\hline
\hline
{\sc \optimathsat{}(fzn+int)}    & 100 &       55 & 42 & 3 & 0 &  7112 & 38 & 1\\
{\sc \optimathsat{}(fzn+bv)}     & 100 & {\bf 57} & 43 & 0 & 0 & 13306 & 30 & 0\\
\hline
{\sc \vbest{}(\optimathsat{})}     & 100 & 68 & 32 & 0 & 0 &  9564 & - & -\\
\hline
\hline
{\sc \vbest{}(all)}              & 100 & 93 &  7 & 0 & 0 &  3657 & - & -\\
\hline
\end{tabularx}%
%\vspace{3ex}
%\scalebox{1.0}{
%    \includegraphics{figs/mzn/mc/cactus_plot.pdf}
%}
\caption[Comparison on the \minizinc{} Challenge 2016 formulas]{
\label{tab:mc16}
A comparison on the performance of \optimathsat{} and various
top-scoring \minizinc{} solvers on the \minizinc{} Challenge 2016 formulas.
%
The columns list the
total number of instances (inst.),
the number of instances solved (termin.),
the number of timeouts (timeout),
the number of unsupported problems (unsup.),
the number of run-time errors (errors),
the total solving time for all solved instances (time),
the number of instances solved in the shortest time within the same category (BT1),
the number of instances solved in the shortest time considering all tools (BT2).
}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> src/tables/mc16_small.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}[tb]
\scriptsize
\centering
\begin{tabularx}{\textwidth}{|X|rcr|rcr|rcr|rcr|rcr|RCR|rcr|rcr|rcr|}
\cline{14-22}
\multicolumn{13}{c}{} &
\multicolumn{9}{|c|}{\bf terminated} &
\multicolumn{6}{c}{} \\
\cline{2-28}
\multicolumn{1}{c|}{} &
\multicolumn{3}{c|}{\bf inst.}     &
\multicolumn{3}{c|}{\bf timeout}   &
\multicolumn{3}{c|}{\bf error}     &
\multicolumn{3}{c|}{\bf unsup.}    &
\multicolumn{3}{c|}{\bf incor.}    &
\multicolumn{3}{c|}{\bf correct}   &
\multicolumn{3}{c|}{\bf time (s.)} &
\multicolumn{3}{c|}{\bf BT1}       &
\multicolumn{3}{c|}{\bf BT2}       \\
\hline
{\bf tool, configuration \& encoding} &
\scsat{} & / & \scopt{} &
\scsat{} & / & \scopt{} &
\scsat{} & / & \scopt{} &
\scsat{} & / & \scopt{} &
\scsat{} & / & \scopt{} &
\scsat{} & / & \scopt{} &
\scsat{} & / & \scopt{} &
\scsat{} & / & \scopt{} &
\scsat{} & / & \scopt{} \\
\hline
%%% INSERT HERE %%%




{\sc picat(cp)} & 15 & / & 85 & 9 &/& 70 & 0 &/& 0 & 0 &/& 0 & 0 &/& 0 & 6 &/& 15 & 2281 &/& 6043 & 0 &/& 0 & 0 &/& 0 \\
{\sc G12()} & 15 & / & 85 & 4 &/& 71 & 1 &/& 3 & 0 &/& 0 & 0 &/& 0 & 10 &/& 11 & 4436 &/& 4220 & 0 &/& 0 & 0 &/& 0 \\
{\sc choco(fixed)} & 15 & / & 85 & 3 &/& 50 & 0 &/& 0 & 0 &/& 0 & 0 &/& 0 & 12 &/& 35 & 4256 &/& 11423 & 1 &/& 0 & 1 &/& 0 \\
{\sc isplus()} & 15 & / & 85 & 6 &/& 44 & 0 &/& 0 & 0 &/& 0 & 0 &/& 0 & 9 &/& 41 & 999 &/& 5492 & 3 &/& 4 & 3 &/& 4 \\
{\sc chuffed()} & 15 & / & 85 & 2 &/& 40 & 0 &/& 0 & 5 &/& 0 & 0 &/& 0 & 8 &/& 45 & 635 &/& 4187 & 0 &/& 5 & 0 &/& 5 \\
{\sc jacop()} & 15 & / & 85 & 3 &/& 39 & 0 &/& 0 & 0 &/& 0 & 0 &/& 0 & 12 &/& 46 & 3411 &/& 12825 & 0 &/& 0 & 0 &/& 0 \\
{\sc ortools(cp)} & 15 & / & 85 & 0 &/& 8 & 0 &/& 0 & 5 &/& 25 & 0 &/& 0 & 10 &/& 52 & 432 &/& 1138 & 0 &/& 27 & 0 &/& 27 \\
{\sc Gurobi()} & 15 & / & 85 & 6 &/& 22 & 0 &/& 0 & 0 &/& 0 & 0 &/& 0 & 9 &/& 63 & 2346 &/& 3037 & 0 &/& 15 & 0 &/& 15 \\
{\sc hcsp()} & 15 & / & 85 & 4 &/& 23 & 0 &/& 0 & 0 &/& 0 & 0 &/& 0 & 11 &/& 62 & 591 &/& 4444 & 0 &/& 10 & 0 &/& 10 \\
{\sc picat(sat)} & 15 & / & 85 & 1 &/& 26 & 0 &/& 0 & 0 &/& 0 & 0 &/& 0 & 14 &/& 59 & 151 &/& 7293 & 10 &/& 1 & 10 &/& 1 \\
{\sc ortools(sat)} & 15 & / & 85 & 1 &/& 15 & 0 &/& 0 & 0 &/& 0 & 0 &/& 0 & 14 &/& 70 & 555 &/& 1338 & 1 &/& 32 & 1 &/& 32 \\
\hline
{\sc virtual best(\minizinc{})} & 15 & / & 85 & 0 &/& 7 & 0 &/& 0 & 0 &/& 0 & 0 &/& 0 & 15 &/& 78 & 146 &/& 3511 & - &/& - & - &/& - \\
\hline\hline
{\sc \optimathsat{}(la)} & 15 & / & 85 & 10 &/& 38 & 0 &/& 0 & 0 &/& 0 & 0 &/& 0 & 5 &/& 47 & 604 &/& 4856 & 1 &/& 20 & 0 &/& 0 \\
{\sc \optimathsat{}(bv)} & 15 & / & 85 & 2 &/& 42 & 0 &/& 0 & 0 &/& 0 & 0 &/& 0 & 13 &/& 43 & 3664 &/& 8561 & 11 &/& 2 & 0 &/& 0 \\
{\sc \bclt{}(la)} & 15 & / & 85 & 10 &/& 33 & 0 &/& 0 & 0 &/& 0 & 0 &/& 0 & 5 &/& 52 & 1117 &/& 5998 & 0 &/& 15 & 0 &/& 2 \\
{\sc \zthree{}(la)} & 15 & / & 85 & 10 &/& 32 & 0 &/& 0 & 0 &/& 0 & 0 &/& 0 & 5 &/& 53 & 676 &/& 10424 & 0 &/& 11 & 0 &/& 0 \\
{\sc \zthree{}(bv)} & 15 & / & 85 & 5 &/& 28 & 0 &/& 0 & 0 &/& 0 & 0 &/& 0 & 10 &/& 57 & 2938 &/& 11113 & 2 &/& 19 & 0 &/& 0 \\
\hline
{\sc virtual best(\omt{})} & 15 & / & 85 & 1 &/& 21 & 0 &/& 0 & 0 &/& 0 & 0 &/& 0 & 14 &/& 64 & 3842 &/& 6432 & - &/& - & - &/& - \\
\hline\hline
{\sc virtual best(all)} & 15 & / & 85 & 0 &/& 7 & 0 &/& 0 & 0 &/& 0 & 0 &/& 0 & 15 &/& 78 & 146 &/& 3511 & - &/& - & - &/& - \\




%%% %%% %%% %%% %%%
\hline
\end{tabularx}
\caption[Comparison on the \minizinc{} Challenge 2016 formulas]{
\label{tab:mc16}
A comparison on the performance of three \omt{} solvers and various
top-scoring \minizinc{} solvers on the \minizinc{} Challenge 2016 formulas.
%
The columns list the
total number of instances (inst.),
the number of timeouts (timeout),
the number of run-time errors (error),
the number of unsupported problems (unsup.),
the number of incorrectly solved instances (incor.),
the number of correctly solved instances (correct),
the total solving time for all solved instances (time),
the number of instances solved in the shortest time within the same category (BT1),
the number of instances solved in the shortest time considering all tools (BT2).
}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> src/tables/mc19_small.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}[tb]
\scriptsize
\centering
\begin{tabularx}{\textwidth}{|X|rcr|rcr|rcr|rcr|rcr|RCR|rcr|rcr|rcr|}
\cline{14-22}
\multicolumn{13}{c}{} &
\multicolumn{9}{|c|}{\bf terminated} &
\multicolumn{6}{c}{} \\
\cline{2-28}
\multicolumn{1}{c|}{} &
\multicolumn{3}{c|}{\bf inst.}     &
\multicolumn{3}{c|}{\bf timeout}   &
\multicolumn{3}{c|}{\bf error}     &
\multicolumn{3}{c|}{\bf unsup.}    &
\multicolumn{3}{c|}{\bf incor.}    &
\multicolumn{3}{c|}{\bf correct}   &
\multicolumn{3}{c|}{\bf time (s.)} &
\multicolumn{3}{c|}{\bf BT1}       &
\multicolumn{3}{c|}{\bf BT2}       \\
\hline
{\bf tool, configuration \& encoding} &
\scsat{} & / & \scopt{} &
\scsat{} & / & \scopt{} &
\scsat{} & / & \scopt{} &
\scsat{} & / & \scopt{} &
\scsat{} & / & \scopt{} &
\scsat{} & / & \scopt{} &
\scsat{} & / & \scopt{} &
\scsat{} & / & \scopt{} &
\scsat{} & / & \scopt{} \\
\hline
%%% INSERT HERE %%%


{\sc choco(std)} & 10 & | & 90 & 4 &|& 63 & 0 &|& 5 & 0 &|& 0 & 0 &|& 0 & 6 &|& 22 & 415 &|& 4312 & 0 &|& 0 & 0 &|& 0 \\
{\sc chuffed() [nightly]} & 10 & | & 90 & 0 &|& 43 & 0 &|& 0 & 5 &|& 10 & 0 &|& 0 & 5 &|& 37 & 1 &|& 4886 & 3 &|& 19 & 3 &|& 19 \\
{\sc G12(std)} & 10 & | & 90 & 5 &|& 64 & 0 &|& 10 & 0 &|& 0 & 0 &|& 0 & 5 &|& 16 & 323 &|& 4010 & 0 &|& 0 & 0 &|& 0 \\
{\sc gecode() [6.2.0]} & 10 & | & 90 & 4 &|& 63 & 0 &|& 0 & 0 &|& 0 & 0 &|& 0 & 6 &|& 27 & 420 &|& 5094 & 0 &|& 6 & 0 &|& 6 \\
{\sc hcsp()} & 10 & | & 90 & 0 &|& 47 & 0 &|& 10 & 0 &|& 0 & 2 &|& 2 & 8 &|& 31 & 2 &|& 6408 & 4 &|& 7 & 4 &|& 4 \\
{\sc iZplus()} & 10 & | & 90 & 5 &|& 71 & 0 &|& 4 & 0 &|& 0 & 0 &|& 0 & 5 &|& 15 & 14 &|& 3077 & 1 &|& 3 & 1 &|& 3 \\
{\sc jacop() [4.8]} & 10 & | & 90 & 4 &|& 55 & 0 &|& 6 & 0 &|& 0 & 0 &|& 0 & 6 &|& 29 & 260 &|& 5467 & 0 &|& 1 & 0 &|& 1 \\
{\sc Gurobi() [8.1.1]} & 10 & | & 90 & 0 &|& 25 & 4 &|& 28 & 0 &|& 0 & 0 &|& 0 & 6 &|& 27 & 1109 &|& 2976 & 1 &|& 6 & 1 &|& 5 \\
{\sc Gurobi(mzn+fzn) [8.1.1]} & 10 & | & 90 & 0 &|& 47 & 0 &|& 9 & 0 &|& 0 & 0 &|& 0 & 10 &|& 34 & 1209 &|& 5118 & 1 &|& 3 & 1 &|& 2 \\
{\sc ortools(sat) [nightly]} & 10 & | & 90 & 5 &|& 42 & 0 &|& 3 & 0 &|& 0 & 0 &|& 0 & 5 &|& 45 & 8 &|& 7239 & 0 &|& 13 & 0 &|& 11 \\
{\sc picat(cp) [2.7b12]} & 10 & | & 90 & 5 &|& 73 & 0 &|& 8 & 0 &|& 0 & 0 &|& 0 & 0 &|& 9 & 0 &|& 2096 & 0 &|& 0 & 0 &|& 0 \\
{\sc picat(sat) [2.7b12]} & 10 & | & 90 & 0 &|& 45 & 0 &|& 5 & 0 &|& 0 & 0 &|& 1 & 10 &|& 39 & 275 &|& 9894 & 0 &|& 7 & 0 &|& 5 \\
\hline{\sc virtual best(\minizinc{})} & 10 & | & 90 & 0 &|& 28 & 0 &|& 0 & 0 &|& 0 & 0 &|& 0 & 10 &|& 62 & 15 &|& 5485 & - &|& - & - &|& - \\
\hline\hline{\sc \optimathsat{}(\smtlib{}+int)} & 10 & | & 90 & 5 &|& 62 & 0 &|& 0 & 0 &|& 0 & 0 &|& 0 & 5 &|& 28 & 4 &|& 3650 & 2 &|& 10 & 0 &|& 0 \\
{\sc \optimathsat{}(\smtlib{}+bv)} & 10 & | & 90 & 4 &|& 59 & 0 &|& 5 & 0 &|& 0 & 0 &|& 0 & 6 &|& 26 & 484 &|& 7271 & 0 &|& 1 & 0 &|& 0 \\
{\sc \bclt{}(\smtlib{}+int)} & 10 & | & 90 & 5 &|& 60 & 0 &|& 0 & 0 &|& 0 & 0 &|& 0 & 5 &|& 30 & 6 &|& 3369 & 0 &|& 6 & 0 &|& 5 \\
{\sc \zthree{}(\smtlib{}+int)} & 10 & | & 90 & 5 &|& 64 & 0 &|& 0 & 0 &|& 0 & 0 &|& 0 & 5 &|& 26 & 4 &|& 5358 & 3 &|& 6 & 0 &|& 1 \\
{\sc \zthree{}(\smtlib{}+bv)} & 10 & | & 90 & 0 &|& 55 & 0 &|& 2 & 0 &|& 0 & 0 &|& 0 & 10 &|& 33 & 1629 &|& 7550 & 5 &|& 17 & 0 &|& 3 \\
\hline{\sc virtual best(\omt{})} & 10 & | & 90 & 0 &|& 48 & 0 &|& 2 & 0 &|& 0 & 0 &|& 0 & 10 &|& 40 & 1624 &|& 5179 & - &|& - & - &|& - \\
\hline\hline{\sc virtual best(all)} & 10 & | & 90 & 0 &|& 28 & 0 &|& 0 & 0 &|& 0 & 0 &|& 0 & 10 &|& 62 & 15 &|& 5051 & - &|& - & - &|& - \\


%%% %%% %%% %%% %%%
\hline
\end{tabularx}
\caption[Comparison on the \minizinc{} Challenge 2019 formulas]{
\label{tab:mc19}
A comparison on the performance of three \omt{} solvers and various
top-scoring \minizinc{} solvers on the \minizinc{} Challenge 2019 formulas.
%
The columns list the
total number of instances (inst.),
the number of timeouts (timeout),
the number of run-time errors (error),
the number of unsupported problems (unsup.),
the number of incorrectly solved instances (incor.),
the number of correctly solved instances (correct),
the total solving time for all solved instances (time),
the number of instances solved in the shortest time within the same category (BT1),
the number of instances solved in the shortest time considering all tools (BT2).
}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> src/tables/omt_reals_merged.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}[tb]
\begin{tabularx}{\textwidth}{|X|r|r|r|r|x|y|r|r|r||r|r|r|r|r|r|}
\cline{5-16}
\multicolumn{4}{c|}{} & \multicolumn{6}{c||}{\bf terminated} & \multicolumn{6}{c|}{\bf incorrect results}\\
\hline
\textbf{tool \& configuration} &
\rotatebox{90}{\textbf{instances}} &
\rotatebox{90}{\textbf{timeout}} &
\rotatebox{90}{\textbf{tool-errors}} &
\rotatebox{90}{\textbf{incorrect}} &
\rotatebox{90}{\textbf{verified}} &
\rotatebox{90}{\textbf{unverified}} &
\rotatebox{90}{\textbf{tot. time (s.)}} &
\rotatebox{90}{\textbf{avg. time (s.)}} &
\rotatebox{90}{\textbf{med. time (s.)}} &
\rotatebox{90}{\textbf{unsat}} &
\rotatebox{90}{$ \Delta \geq 10^{-6} $} &
\rotatebox{90}{$ \Delta \geq 10^{-3} $} &
\rotatebox{90}{$ \Delta \geq 10^{-1} $} &
\rotatebox{90}{$ \Delta \geq 10^{0} $} &
\rotatebox{90}{$ \Delta \geq 10^{1} $} \\

\hline\hline
\multicolumn{16}{|c|}{\cellcolor{black!15}\textbf{SAL, Symba, Jobshop and Strippacking}} \\
\hline
    \gecode{}() & 2888 & 2733 & 0 & 0 & 155 & 0 & 10800 & 69.68 & 18.63 & 0 & 0 & 0 & 0 & 0 & 0 \\
    \gmip{} & 2888 & 10 & 0 & 2855 & 0 & 23 & 317 & 13.79 & 11.21 & 2765 & 90 & 90 & 86 & 39 & 0 \\
    \gurobi{}() & 2888 & 48 & 0 & 2728 & 104 & 8 & 3961 & 35.37 & 2.14 & 2684 & 44 & 32 & 32 & 1 & 0 \\
\hline
    \vbestpar{\minizinc{}} & 2888 & 0 & 0 & 2628 & 237 & 23 & 13801 & 53.08 & 6.97 & - & - & - & - & - & - \\
\hline\hline
    \optimfzn{} & 2888 & 31 & 0 & 0 & 2854 & 3 & 22320 & 7.81 & 0.40 & 0 & 0 & 0 & 0 & 0 & 0 \\
\hline
    \vbestpar{fzn} & 2888 & 0 & 0 & 11 & 2854 & 23 & 20674 & 7.19 & 0.40 & - & - & - & - & - & - \\
\hline\hline
    \optimsmt{} & 2888 & 23 & 0 & 0 & \textcolor{blue}{\textbf{2865}} & 0 & 15676 & 5.47 & 0.08 & 0 & - & - & - & - & - \\
\hline\hline
    \vbestpar{all}            &  2888 & 0 & 0 & 0 & 2865 & 23 & 15183 & 5.26 & 0.08 & - & - & - & - & - & - \\
\hline\hline
\multicolumn{16}{|c|}{\cellcolor{black!15}\textbf{Machine Learning}} \\
\hline
    \gecode{}() & 510 & 322 & 0 & 164 & 24 & 0 & 11 & 0.44 & 0.43 & 147 & 17 & 17 & 2 & 0 & 0 \\
    \gmip{} & 510 & 108 & 0 & 400 & 2 & 0 & 225 & 112.47 & 112.47 & 400 & 0 & 0 & 0 & 0 & 0 \\
    \gurobi{}() & 510 & 9 & 0 & 472 & 28 & 1 & 201 & 6.92 & 3.17 & 468 & 4 & 4 & 2 & 0 & 0 \\
\hline
    \vbestpar{\minizinc{}} & 510 & 9 & 0 & 464 & 36 & 1 & 383 & 10.34 & 0.46 & - & - & - & - & - & - \\
\hline\hline
%    \optimfzn & 510 & 298 & 0 & 177 & 35 & 0 & 32 & 0.92 & 0.88 & 177 & 0 & 0 & 0 & 0 & 0 \\
    \optimfzn & 510 & 7 & 0 & 237 & 263 & 3 & 2797 & 10.52 & 2.21 & 177 & 60 & 59 & 0 & 0 & 0 \\
    \optimfzne & 510 & 92 & 0 & 0 & 415 & 3 & 1197 & 2.86 & 2.03 & 0 & 0 & 0 & 0 & 0 & 0 \\
\hline
    \vbestpar{fzn} & 510 & 7 & 0 & 83 & 417 & 3 & 1366 & 3.25 & 2.03 & - & - & - & - & - & - \\
\hline\hline
    \optimsmt & 510 & 10 & 0 & 0 &\textcolor{blue}{\textbf{500}} & 0 & 5766 & 11.53 & 12.15 & 0 & - & - & - & - & - \\
\hline\hline
    \vbestpar{all} & 510 & 7 & 0 & 0 & 500 & 3 & 2290 & 4.55 & 2.05 & - & - & - & - & - & - \\
\hline
\end{tabularx}
\caption{\label{tab:reals}
\omt Problem defined over the rationals.
%
The configuration \optimfzne{} uses the \emzntofzn{} compiler
to translate \minizinc{} into \flatzinc{}.
%
A \satres result is marked as {\em correct} when the objective
value matches the reference solution provided by \optimsmt{}
with an absolute error $\Delta < 10^{-6}$.
%
A result is marked as {\em unverified} when we have
no reference solution.
%
A result is marked as {\em incorrect} if neither
of the previous two conditions apply.
}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

